Study of Initial and Final State Effects in Ultrarelativistic Heavy Ion Collisions Using Hadronic Probes

It has been theorized that if heavy nuclei (e.g. Au, Pb) are collided at sufficiently high energies, we might be to recreate the conditions that existed in the universe a few microseconds after the Big Bang. The kinetic energy of the colliding nuclei gets converted into heat, leading to a phase transition into a new state of matter: the Quark-Gluon Plasma (QGP), in which quarks and gluons are deconfined. However, we never directly get to see the QGP because as the matter cools it recombines (hadronizes) into ordinary subatomic particles. We can only hope to infer its existence from indirect experimental signatures, after hadronization. In this dissertation we attempt to shed some light on: Properties of the final state of produced matter in Au+Au collisions at $\sqrt{s_{NN}}=200$ GeV. As the hot, dense system of particles from the collision zone cools and expands, light nuclei like deuterons and anti-deuterons can be formed, with a probability proportional to the product of the phase space densities of its constituent nucleons. Thus, invariant yield of deuterons, compared to the protons and neutrons from which they coalesce, provides information about the size of the emitting system and its space-time evolution. The initial conditions that led to this. This is done by looking at the nuclear modification factor $R_{cp}$ from particle production in forward and backward directions in a ``control'' experiment using d+Au collisions at $\sqrt{s_{NN}}=200$ GeV. This can allow us to distinguish between effects that could potentially be due to deconfinement, versus effects of cold nuclear matter.

==> abstract_old.tex <==

It has been theorized that if heavy nuclei (e.g. Au, Pb) are collided at sufficiently high energies, we might be to recreate the conditions that existed in the universe a few microseconds after the Big Bang. The kinetic energy of the colliding nuclei gets converted into heat, leading to a phase transition into a new state of matter: the Quark-Gluon Plasma (QGP), in which quarks and gluons are deconfined. However, we never directly get to see the QGP because as the matter cools it recombines (hadronizes) into ordinary subatomic particles. We can only hope to infer its existence from indirect experimental signatures, after hadronization. In this dissertation we attempt to shed some light on:
\benn
\item Properties of the final state of produced matter in Au+Au collisions at $\sqrt{s_{NN}}=200$ GeV. As the hot, dense system of particles from the collision zone cools and expands, light nuclei like deuterons and anti-deuterons can be formed, with a probability proportional to the product of the phase space densities of its constituent nucleons. Thus, invariant yield of deuterons, compared to the protons and neutrons from which they coalesce, provides information about the size of the emitting system and its space-time evolution. 

The transverse momentum spectra of $d$ and $\bar{d}$ in the
range $1.1<p_T<4.3$~GeV/$c$ were measured at mid-rapidity and were found to 
be less steeply falling than proton (and antiproton) spectra. 
A coalescence analysis comparing the deuteron
and antideuteron spectra with that of proton and antiproton was performed and
the extracted coalescence parameter $B_2$ was found to increase with $p_T$, 
indicating an expanding source. 

\item The initial conditions that led to this. This is done by looking at the nuclear modification factor $R_{cp}$ from particle production in forward and backward directions in a ``control'' experiment using d+Au collisions at $\sqrt{s_{NN}}=200$ GeV. This can allow us to distinguish between effects that could potentially be due to deconfinement, versus effects of cold nuclear matter.

We found hadron $R_{cp}$ to be suppressed at forward rapidities
(d going direction). This is qualitatively consistent with 
shadowing/saturation type effects in the small-$x$ region being probed at 
forward rapidities. $R_{cp}$ was enhanced at backward rapidities (Au going 
region). 

==> ack.tex <==
\thispagestyle{empty}
\vspace*{3cm}
\bcc
{\Large{\bf Acknowledgements}}
\ecc
First, of all I would like to acknowledge my advisor Tom Hemmick for
his guidance and support through the ups and the downs of Ph.D research.
His infectious enthusiasm for physics was very inspiring. Ph.D supervison 
under Tom Hemmick, reminds me of the following story:

{\it One sunny day a rabbit came out of her hole in
the ground to enjoy the fine weather. The day
was so nice that she became careless and a
fox sneaked up behind her and caught her.

"I am going to eat you for lunch!", said the fox.

"Wait!" replied the rabbit, "You should at least
wait a few days."

"Oh yeah? Why should I wait?"

"Well, I am just finishing my thesis on 'The
Superiority of Rabbits over Foxes and Wolves.'"

"Are you crazy? I should eat you right now!
Everybody knows that a fox will always win
over a rabbit."

"Not really, not according to my research. If you
like, you can come into my hole and read it for
yourself. If you are not convinced, you can go
ahead and have me for lunch."

"You really are crazy!"   But since the fox was
curious and had nothing to lose, it went with the
rabbit. The fox never came out.  A few days later
the rabbit was again taking a break from writing
and sure enough, a wolf came out of the bushes
and was ready to set upon her.

"Wait!" yelled the rabbit, "you can't eat me right now."

"And why might that be, my furry appetizer?"

"I am almost finished writing my thesis on 'The
Superiority of Rabbits over Foxes and Wolves.'"

The wolf laughed so hard that it almost lost its grip
on the rabbit. "Maybe I shouldn't eat you; you really
are sick--in the head.  You might have something
contagious."

"Come and read it for yourself; you can eat me
afterward if you disagree with my conclusions."

So the wolf went down into the rabbit's hole and
never came out. The rabbit finished her thesis and
was out celebrating in the local lettuce patch. Another
rabbit came along and asked, "What's up? You seem
very happy."

"Yup, I just finished my thesis."

"Congratulations. What's it about?"

"The Superiority of Rabbits over Foxes and Wolves.'"

"Are you sure? That doesn't sound right."

"Oh yes. Come and read it for yourself."

So together they went down into the rabbit's hole.
As they entered, the friend saw the typical graduate
abode, albeit a rather messy one after writing a thesis..
The computer with the controversial work was in one
corner. And to the right there was a pile of fox bones,
on the left a pile of wolf bones.  And in the middle was
a large, well-fed lion.

The moral of the story:
The title of your thesis doesn't matter.
The subject doesn't matter.
The research doesn't matter.
All that matters is who your advisor is.}

The group
at Stony Brook is like a large family. 


all the people with whose
encouragement I embarked upon this career --- my parents and brother and sister, who nurtured 
my interest in science, when I was young as well as authors of popular
science books like . 
 Overall, the years that I have spent here at Stony Brook, have been
some of the most satisfying --- both academically as well as non-academically.
\\
And finally Victor Weisskopf once said:

   {\it There are three kinds of physicists, as we know, namely the machine 
builders, the experimental physicists, and the theoretical physicists. If we 
compare those three classes, we find that the machine builders are the most 
important ones, because if they were not there, we could not get to this 
small-scale region. If we compare this with the discovery of America, then, I 
would say, the machine builders correspond to the captains and ship builders 
who really developed the techniques at that time. The experimentalists were 
those fellows on the ships that sailed to the other side of the world and then
jumped upon the new islands and just wrote down what they saw. The 
theoretical physicists are those fellows who stayed back in Madrid and told 
Columbus that he was going to land in India.}

	This dissertation and the corresponding research would not have been
possible the work done by the 



\newpage


==> appendb.tex <==
\appendix{Parametrizations of the cross sections}

\section{First approach}

The recipe of A.A.Moiseev and J.F.Ormes in Astroparticle Physics 6(1997) 379-386, 
for calculating inelastic anti-helium cross sections on nuclei, can be modified to 
give anti-deuteron cross sections. A.A.Moiseev and J.F.Ormes used their calculations 
to estimate the probability to observe anti-helium among the cosmic rays.

Helium cross sections are parameterized as

\begin{equation}
\sigma_{He,A} = ( 2 \cdot \sigma_{p,A}^{3/2} + 2 \cdot \sigma_{n,A}^{3/2} )^{2/3}  \cdot K_{a}(A)
\label{viktig}
\end{equation}

where $\sigma_{p,A}$ and $\sigma_{n,A}$ are the inelastic cross sections for protons and 
neutrons on nuclei, respectively. (It is not easy to see the idea behind this parameterization.)
 
In our case we will instead have

\begin{equation}
\sigma_{d,A} = ( \sigma_{p,A}^{3/2} + \sigma_{n,A}^{3/2} )^{2/3} \cdot K_{d}(A)
\end{equation}

The following parameterizations of $\sigma_{p,A}$ and $\sigma_{n,A}$ are used by the authors:

\begin{equation}
\sigma_{p,A}(E) = 45 \cdot A^{0.7} \cdot [1 + 0.016 \sin(5.3 - 2.63 \ln A )] \cdot 
[1 - 0.62 \exp(-5E) \sin(1.58 \cdot E^{-0.28})] 
\end{equation}

and 

\begin{equation}
\sigma_{n,A} = (43.2 \pm 2.3) \cdot A^{0.719 \pm 0.012} 
\end{equation}

In the proton case E is the kinetic energy of the proton in GeV and the cross sections are 
given in mb. For the proton case 45$A^{0.7}$ can be used above 0.8 GeV.

Based on experimental data they find

\begin{equation}
K_{a}(A) = 1.2 \cdot [ \ln (A + 2)]^{-0.5} 
\end{equation}

Using available data on deuteron induced interactions

\begin {table} [H] \begin{center} 
\begin{small}
\begin{tabular} { l l l } \hline 
Projectile & $\sigma$ [mb] & Reference \\ \hline
$^2$d      & 134   & \cite{Jaros}          \\   
$^4$He     & 204   & \cite{Abdurak}        \\ 
$^{12}$C   & 401   & \cite{Jaros,Abdurak}  \\  
$^{181}$Ta & 1940  & \cite{Abdurak}        \\ \hline
\end{tabular}
\end{small}
\caption{Deuteron induced cross section with nuclei.}
\end{center} \end{table}

we find a similar expression for $K_d(A)$, namely

\begin{equation}
K_{d}(A) = 1.6 \cdot [\ln (A + 4)]^{-0.5} 
\end{equation}

In the paper it is assumed that the anti-helium cross sections can be written 
in the same way as in Eq.~\ref{viktig}, i.e.

\begin{equation}
\sigma_{\overline{He},A} = (2 \cdot \sigma_{\overline{p},A}^{3/2} + 2 \cdot \sigma_{\overline{n},A}^{3/2} )^{2/3} 
\cdot K_{\alpha}(A) 
\end{equation}

where it is assumed that the factor $K_{\alpha}(A)$ is the same as in 
Eq.~\ref{viktig}. (This assumption 
is also questionable, since this factor contains most of the mass dependence.)

In the deuteron case we will similarly be able to write

\begin{equation}
\sigma_{\overline{d},A} = ( \sigma_{\overline{p},A}^{3/2} + \sigma_{\overline{n},A}^{3/2} )^{2/3} \cdot K_{d}(A)
\end{equation}

The following parameterizations of $\sigma_{\overline{p},A}$ and $\sigma_{\overline{n},A}$ are used 
by the authors:

\begin{equation}
\sigma_{\overline{p},A} = A^{2/3} \cdot \left[ 48.2 + 19 \cdot (E - 0.02)^{-0.55} 
   - 0.106 \cdot A^{0.927} \cdot E^{-1.2} 
   + 0.059 A^{0.927} + 0.00042 A^{1.854} \cdot E^{-1.5} \right]
\end{equation}

and

\begin{equation}
\sigma_{\overline{n},A} = A^{2/3} \cdot ( 51 + 16 \cdot E^{-0.4} ) 
\end{equation}


\section{A new approach}

The idea behind Eq.~\ref{viktig} is however not transparent. There is no real picture 
behind this parameterization. Furthermore, since the factor K$_{\alpha}$(A) contains 
most of the mass dependence (and even has to compensate for the wrong mass 
dependence introduced by Eq.~\ref{viktig}), it is not at all evident that this factor 
will be the same in the anti-helium (anti-deuteron) case.  

\begin{figure}[htb]
    \includegraphics[angle=270,width=16cm]{figures/traffbild.eps}
    \label{traffbild}
    \caption{Geometric motivation for the second approach.}
\end{figure}

A different approach would be to start with

\begin{equation}
\sigma_{He,A} = \sigma_{N,A} +  \Delta \sigma_{He,A} 
\end{equation}

where

\begin{equation}
\sigma_{N,A} = \frac{\sigma_{p,A} + \sigma_{n,A}}{2}
\end{equation}

Now, from the figure above, we obtain

\begin{equation}
\sigma_{He,A} = \left[  \sqrt{ \sigma_{N,A} } + \Delta_{He}(A)  \right]^2  
\end{equation}

from which we find

\begin{equation}
\Delta_{He}(A) = \sqrt{ \sigma_{He,A} } - \sqrt{ \sigma_{N,A} } 
\end{equation}

From experimental data we find $\Delta_{He} = 6.03 \pm 0.23$, independent of $A$, 
within the experimental errors.

For deuterons we obtain similarly

\begin{equation}
\sigma_{d,A} = \left[ \sqrt{\sigma_{N,A}} + \Delta_{d}(A)  \right]^2 
\end{equation}

and

\begin{equation}
\Delta_{d}(A) = \sqrt{ \sigma_{d,A} } - \sqrt{ \sigma_{N,A} } 
\end{equation}

Again we use experimental data to find $\Delta_{d} = 3.51 \pm 0.25$ independent of $A$.

For $\sigma_{\overline{He},A}$ and $\sigma_{\overline{d},A}$ we use the idea of A.A.Moiseev and J.F.Ormes 
and write

\begin{equation}
\sigma_{\overline{He},A} = \left[  \sqrt{\sigma_{N,A}} + \Delta_{He}  \right]^2 
\end{equation}

and

\begin{equation}
\sigma_{\overline{d},A} = \left[  \sqrt{\sigma_{\overline{N},A}} + \Delta_{d}  \right]^2 
\end{equation}

where

\begin{equation}
\sigma_{\overline{N},A} = \frac{\sigma_{\overline{p},A} + \sigma_{\overline{n},A}}{2}
\end{equation}

In this case it is much more plausible to use the same terms $\Delta_{He}$ and $\Delta_d$, since these 
terms only reflect the difference in size between a Helium-nucleus (deuteron) and a 
proton, and this difference in size should be the same if anti-nuclei and 
anti-protons are compared. Furthermore they show no mass dependence.

Care should be taken when the paramterizations are used at the lowest energies.

==> appendc.tex <==
\appendix{Media and materials in Pisa}

\begin {table} [H] \begin{center} 
\begin{tiny}
\begin{tabular} { l l l r} \hline 
MEDIUM  & NAME                   &     MATERIAL & Length $[cm]$ \\ \hline
\multicolumn{4}{c}{General} \\
      1 & HELIUM                 &     3        & 174.267 \\
      6 & AIR                    &    15        &   0.365 \\
     10 & Silicon                &    50        &   0.014 \\
     18 & AIRLOWF                &    15        &  18.081 \\
     19 & AIRF                   &    15        &  34.205 \\
     24 & MPC FRAME              &    72        &   0.332 \\
     25 & MPC MYLR PLN           &    73        &   0.026 \\
     26 & Aluminum Frame         &     9        &   0.054 \\
\multicolumn{4}{c}{Beam-pipe} \\
     33 & Be + Field             &     5        &   0.103 \\
\multicolumn{4}{c}{MVD} \\
    101 & NSilicon               &    50        &   0.002 \\
    102 & Rohacell               &   102        &   1.349 \\
    105 & Silicon                &    50        &   0.028 \\
    106 & MVD Aluminum           &     9        &   0.006 \\
    108 & MVD cable              &   108        &   0.004 \\
\multicolumn{4}{c}{Drift Chamber} \\
    415 & DC Window              &   463        &   0.020 \\
    465 &  GAS IN DR CH 1        &   466        &  32.488 \\
    480 &  ACT GAS IN DR CH 1    &   466        &  12.144 \\
\multicolumn{4}{c}{PC1} \\
    490 & CARBON-FIBER/EPOXY     &   490        &   0.028 \\
    491 & S2-GLASS/EPOXY         &   491        &   0.026 \\
    492 & HEXCELL CORE           &   492        &   5.139 \\
    493 & EPOXY GLUE             &   493        &   0.020 \\
    494 & PAD CHAMBER GAS        &   494        &   0.607 \\
    495 & PAD CATHODE BOARD      &   495        &   0.026 \\
    496 & GROUND CATHODE BOARD   &   496        &   0.026 \\
    497 & MOTHER BOARD           &   497        &   1.014 \\
\multicolumn{4}{c}{RICH} \\
    503 & CO2                    &   503        & 149.005 \\
    511 & RICH MIR. SUBSTRATE    &   511        &   1.176 \\
\multicolumn{4}{c}{TEC} \\
    680 & AIR                    &   680        &  42.635 \\
    682 & G10                    &   682        &   0.058 \\
    685 & XEA                    &   685        &  21.526 \\
    686 & XEN                    &   686        &   0.607 \\
    687 & MYL                    &   687        &   0.088 \\
    688 & GRA                    &   688        &   0.255 \\
\multicolumn{4}{c}{PC3} \\
    690 & CARBON-FIBER/EPOXY     &   690        &   0.055 \\
    691 & S2-GLASS/EPOXY         &   691        &   0.142 \\
    692 & HEXCELL CORE           &   692        &   4.464 \\
    695 & PAD CATHODE BOARD      &   695        &   0.037 \\
    696 & GROUND CATHODE BOARD   &   696        &   0.058 \\
    697 & MOTHER BOARD           &   697        &   0.549 \\
    699 & PC3 CHAMBER GAS        &   694        &   0.872 \\
\multicolumn{4}{c}{Time-of-Flight} \\
    706 & TOF Carbon             &     6        &   0.631 \\ \hline
\end{tabular}
\end{tiny}
\caption{Tracking media traversed by geantinos in the East PHENIX tracking arm 
with corresponding path lengths.}
\label{trmedia}
\end{center} \end{table}



\begin {table} [H] \begin{center} 
\begin{tiny}
\begin{tabular} { l l r r l l l l r r l} \hline 
MTRL      & NAME                 &    A      &   Z     & $\rho$  & RADIAT L  & ABSORP L  & NMIX &     &       &        \\ 
          &                      &           &         & [g/cm$^3$] & [cm]   & [cm]      &      &     &       &        \\\hline
        3 & HELIUM (GAS)         &   4.000   &   2.000 &  0.0002 & 0.530E+06 & 0.336E+06 &  1 &        &       &       \\
        5 & BERILLIUM            &   9.010   &   4.000 &   1.848 & 0.353E+02 & 0.367E+02 &  1 &        &       &       \\
        6 & CARBON               &  12.010   &   6.000 &   2.265 & 0.188E+02 & 0.499E+02 &  1 &        &       &       \\
        9 & ALUMINIUM            &  26.980   &  13.000 &   2.700 & 0.890E+01 & 0.372E+02 &  1 &        &       &       \\
       15 & AIR                  &  14.610   &   7.300 &   0.001 & 0.304E+05 & 0.675E+05 &  1 &        &       &       \\
       50 & SILICON              &  28.090   &  14.000 &   2.330 & 0.936E+01 & 0.455E+02 &  1 &        &       &       \\
       72 & TOF PMT Base         &  18.140   &   9.065 &   1.700 & 0.194E+02 & 0.567E+02 &  1 &        &       &       \\
       73 & MYLAR                &  12.880   &   6.456 &   1.390 & 0.287E+02 & 0.561E+02 &  1 &        &       &       \\
      102 &  ROHACELL            &  12.230   &   6.147 &   0.075 & 0.543E+03 & 0.125E+04 &  4 &   A    &  Z    & W     \\
          &                      &           &         &         &           &           &    &   1.01 &  1.00 & 0.072 \\
          &                      &           &         &         &           &           &    &  12.01 &  6.00 & 0.627 \\
          &                      &           &         &         &           &           &    &  14.01 &  7.00 & 0.091 \\
          &                      &           &         &         &           &           &    &  16.00 &  8.00 & 0.209 \\
      108 & MVD cables           &  30.633   &  14.346 &   2.163 & 0.106E+02 & 0.522E+02 &  5 &   A    &  Z    & W     \\
          &                      &           &         &         &           &           &    &  12.01 &  6.00 & 0.447 \\
          &                      &           &         &         &           &           &    &  14.01 &  7.00 & 0.047 \\
          &                      &           &         &         &           &           &    &  16.00 &  8.00 & 0.135 \\
          &                      &           &         &         &           &           &    &   1.01 &  1.00 & 0.017 \\
          &                      &           &         &         &           &           &    &  63.54 & 29.00 & 0.353 \\
      463 &   MYLAR              &  12.872   &   6.456 &   1.390 & 0.286E+02 & 0.700E+02 &  3 &   A    &  Z    & W     \\
          &                      &           &         &         &           &           &    &  12.01 &  6.00 & 0.625 \\
          &                      &           &         &         &           &           &    &   1.01 &  1.00 & 0.042 \\
          &                      &           &         &         &           &           &    &  15.99 &  8.00 & 0.333 \\
      466 & DC GAS               &  21.855   &  10.125 &   0.001 & 0.275E+05 & 0.779E+05 &  3 &   A    &  Z    & W     \\
          &                      &           &         &         &           &           &    &  39.95 & 18.00 & 0.500 \\
          &                      &           &         &         &           &           &    &  12.01 &  6.00 & 0.125 \\
          &                      &           &         &         &           &           &    &   1.01 &  1.00 & 0.375 \\
      490 & G10                  &  18.140   &   9.065 &   1.700 & 0.194E+02 & 0.567E+02 &  1 &        &       &       \\
      491 & G10                  &  18.140   &   9.065 &   1.700 & 0.194E+02 & 0.567E+02 &  1 &        &       &       \\
      492 & HEXCELL              &  12.010   &   6.000 &   0.024 & 0.817E+04 & 0.100E+06 &  1 &        &       &       \\
      493 & EPOXY GLUE           &  18.140   &   9.065 &   1.700 & 0.194E+02 & 0.567E+02 &  1 &        &       &       \\
      494 & PAD CHAMBER GAS      &  21.855   &  10.125 &   0.001 & 0.275E+05 & 0.779E+05 &  3 &   A    &  Z    & W     \\
          &                      &           &         &         &           &           &    &  39.95 & 18.00 & 0.500 \\
          &                      &           &         &         &           &           &    &  12.01 &  6.00 & 0.125 \\
          &                      &           &         &         &           &           &    &   1.01 &  1.00 & 0.375 \\
      495 & CATHODE BOARD        &  18.866   &   9.384 &   1.820 & 0.166E+02 & 0.610E+02 &  2 &   A    &  Z    & W     \\
          &                      &           &         &         &           &           &    &  18.14 &  9.06 & 0.984 \\
          &                      &           &         &         &           &           &    &  63.54 & 29.00 & 0.016 \\
      496 & GROUND CATHODE BOARD &  18.866   &   9.384 &   1.820 & 0.166E+02 & 0.610E+02 &  2 &   A    &  Z    & W     \\
          &                      &           &         &         &           &           &    &  18.14 &  9.06 & 0.984 \\
          &                      &           &         &         &           &           &    &  63.54 & 29.00 & 0.016 \\
      497 & MOTHER BOARD         &  14.827   &   7.406 &   0.093 & 0.390E+03 & 0.112E+04 &  3 &   A    &  Z    & W     \\
          &                      &           &         &         &           &           &    &  18.14 &  9.06 & 0.050 \\
          &                      &           &         &         &           &           &    &  63.54 & 29.00 & 0.001 \\
          &                      &           &         &         &           &           &    &  14.61 &  7.30 & 0.949 \\
      503 & CO2                  &  14.911   &   7.454 &   0.002 & 0.184E+05 & 0.532E+05 &  2 &   A    &  Z    & W     \\
          &                      &           &         &         &           &           &    &  12.01 &  6.00 & 0.273 \\
          &                      &           &         &         &           &           &    &  16.00 &  8.00 & 0.727 \\
      511 & RICH MIR. SUBSTRATE  &  11.856   &   5.954 &   0.290 & 0.144E+03 & 0.325E+03 &  4 &   A    &  Z    & W     \\
          &                      &           &         &         &           &           &    &   1.01 &  1.00 & 0.061 \\
          &                      &           &         &         &           &           &    &  12.01 &  6.00 & 0.776 \\
          &                      &           &         &         &           &           &    &  14.01 &  7.00 & 0.067 \\
          &                      &           &         &         &           &           &    &  16.00 &  8.00 & 0.096 \\
      680 & AIR                  &  14.610   &   7.300 &   0.001 & 0.304E+05 & 0.675E+05 &  1 &        &       &       \\
      682 & G10                  &  20.000   &  10.000 &   1.700 & 0.194E+02 & 0.536E+02 &  1 &        &       &       \\
      685 & 50\%Xe+50\%He        & 127.527   &  52.463 &   0.003 & 0.287E+04 & 0.596E+05 &  2 &   A    &  Z    & W     \\
          &                      &           &         &         &           &           &    & 131.29 & 54.00 & 0.970 \\
          &                      &           &         &         &           &           &    &   4.00 &  2.00 & 0.030 \\
      686 & 50\%Xe+50\%He        & 131.172   &  53.952 &   0.003 & 0.280E+04 & 0.623E+05 &  2 &   A    &  Z    & W     \\
          &                      &           &         &         &           &           &    & 131.29 & 54.00 & 0.999 \\
          &                      &           &         &         &           &           &    &   4.00 &  2.00 & 0.001 \\
      687 & MYLAR                &  12.872   &   6.456 &   1.390 & 0.286E+02 & 0.700E+02 &  3 &   A    &  Z    & W     \\
          &                      &           &         &         &           &           &    &  12.01 &  6.00 & 0.625 \\
          &                      &           &         &         &           &           &    &   1.01 &  1.00 & 0.042 \\
          &                      &           &         &         &           &           &    &  15.99 &  8.00 & 0.333 \\
      688 & Graph/Epoxy          &  12.011   &   6.000 &   1.680 & 0.250E+02 & 0.990E+02 &  1 &        &       &       \\
      690 & G10                  &  18.140   &   9.065 &   1.700 & 0.194E+02 & 0.567E+02 &  1 &        &       &       \\
      691 & G10                  &  18.140   &   9.065 &   1.700 & 0.194E+02 & 0.567E+02 &  1 &        &       &       \\
      692 & HEXCELL              &  12.010   &   6.000 &   0.024 & 0.817E+04 & 0.100E+06 &  1 &        &       &       \\
      694 & PAD CHAMBER GAS      &  21.855   &  10.125 &   0.001 & 0.275E+05 & 0.779E+05 &  3 &   A    &  Z    & W     \\
          &                      &           &         &         &           &           &    &  39.95 & 18.00 & 0.500 \\
          &                      &           &         &         &           &           &    &  12.01 &  6.00 & 0.125 \\
          &                      &           &         &         &           &           &    &   1.01 &  1.00 & 0.375 \\
      695 & CATHODE BOARD        &  19.593   &   9.703 &   1.930 & 0.153E+02 & 0.578E+02 &  2 &   A    &  Z    & W     \\
          &                      &           &         &         &           &           &    &  18.14 &  9.06 & 0.968 \\
          &                      &           &         &         &           &           &    &  63.54 & 29.00 & 0.032 \\
      696 & GROUND CATHODE BOARD &  18.866   &   9.384 &   1.820 & 0.166E+02 & 0.610E+02 &  2 &   A    &  Z    & W     \\
          &                      &           &         &         &           &           &    &  18.14 &  9.06 & 0.984 \\
          &                      &           &         &         &           &           &    &  63.54 & 29.00 & 0.016 \\
      697 & MOTHER BOARD         &  14.827   &   7.406 &   0.093 & 0.390E+03 & 0.112E+04 &  3 &   A    &  Z    & W     \\
          &                      &           &         &         &           &           &    &  18.14 &  9.06 & 0.050 \\
          &                      &           &         &         &           &           &    &  63.54 & 29.00 & 0.001 \\
          &                      &           &         &         &           &           &    &  14.61 &  7.30 & 0.949 \\ \hline
\end{tabular}
\end{tiny}
\caption{Pisa material definitions for the tracking media listed in the previous table.}
\label{trmaterial}
\end{center} \end{table}












==> appendd.tex <==
\section{Appendix D}

\begin{table}
\caption[]{{\bf Raw Yields for min. bias events} 
(File: {\it ppg020_0_92_final.txt})}
\begin{tabular}[ ]{lll}
\hline
$p_T$ GeV& Raw counts for $d$ &  Raw counts for $\bar{d}$ \\
\hline
1.3	&	690.712	$\pm$	49.868	&	322.114	$\pm$	26.9392	\\
1.7	&	782.783	$\pm$	35.6892	&	412.272	$\pm$	29.811	\\
2.1	&	760.001	$\pm$	32.999	&	336.306	$\pm$	24.556	\\
2.5	&	477.309	$\pm$	27.9426	&	199.812	$\pm$	20.3159	\\
2.9	&	229.359	$\pm$	23.4378	&	112.669	$\pm$	17.5777	\\
3.3	&	133.208	$\pm$	18.8056	&	71.6043	$\pm$	14.913	\\
3.9	&	69.7416	$\pm$	21.3508	&	58.9473	$\pm$	20.2146	\\
\hline
\end{tabular}
\label{tab:raw2}
\end{table}


\begin{table}
\caption[]{{\bf Raw Yields for 0-20\% centrality events} 
(File: {\it ppg020_0_20_final.txt})}
\begin{tabular}[ ]{lll}
\hline
$p_T$ GeV& Raw counts for $d$ &  Raw counts for $\bar{d}$ \\
\hline
1.3	&	378.291	$\pm$	31.4306	& 171.522 $\pm$ 21.9933		\\
1.7	&	443.66	$\pm$	28.3072	&	210.57 $\pm$ 20.5607		\\
2.1	&	449.276	$\pm$	26.1366	&	207.874$\pm$  20.1791		\\
2.5	&	308.455	$\pm$	23.2434	&	116.245 $\pm$ 16.7561		\\
2.9	&	145.113	$\pm$	19.6931	&	75.9248 $\pm$ 14.242		\\
3.3	&	72.1734	$\pm$	14.8395	&	46.3732 $\pm$ 12.3767		\\
3.9	&	50.032	$\pm$	18.0059	&	40.9745 $\pm$ 15.8305		\\
\hline
\end{tabular}
\label{tab:raw0}
\end{table}


\begin{table}
\caption[]{{\bf Raw Yields for 20-92\% centrality events} 
(File: {\it ppg020_20_92_final.txt})}
\begin{tabular}[ ]{lll}
\hline
$p_T$ GeV& Raw counts for $d$ &  Raw counts for $\bar{d}$ \\
\hline
1.3	&	314.905	$\pm$	24.9601	&	153.976	$\pm$	15.5005	\\
1.7	&	338.779	$\pm$	21.5489	&	203.035	$\pm$	16.7537	\\
2.1	&	313.051	$\pm$	20.1975	&	129.831	$\pm$	13.8321	\\
2.5	&	177.778	$\pm$	16.5595	&	76.1233	$\pm$	11.838	\\
2.9	&	87.5999	$\pm$	13.9707	&	39.7836	$\pm$	10.2824	\\
3.3	&	70.3182	$\pm$	13.1204	&	31.136	$\pm$	8.79026	\\
3.9	&	31.368	$\pm$	13.1671	&	17.3637	$\pm$	11.5297	\\
\hline
\end{tabular}
\label{tab:raw1}
\end{table}


==> appende.tex <==
\section{Appendix E}
For a Boltzman distribution:
\[
E\frac{d^3N}{dp^3} = Ee^{-E/T_{eff}}
\]
or since $E = m_T\cosh(y)$ we get:
\[
\frac{d^2N}{2\pi N_{evt}m_tdm_tdy} = m_T\cosh(y)e^{-m_t\cosh(y)/T_{eff}}
\]
Since for Phenix, we are in a mid-rapidity slice, $\cosh(y=0) = 1$, and
we get
\[
\frac{d^2N}{2\pi N_{evt}m_tdm_tdy}\vline\ _{y=0} = m_Te^{-m_t/T_{eff}}
\]
which is the correct form. However, if we integrate over y, we get the
form:
\[
\frac{dN}{2\pi N_{evt}m_tdm_t} \propto \sqrt{m_T}e^{-m_t/T_{eff}}
\]
which has been used historically and is incorrect, since at Phenix, we measure
only over a limited slice of rapidity.



==> cpt_faq_akp_phd.tex <==
\chapter{FAQs}

\section{Some jargon}
\benn
\item 

\eenn
\section{Invariant yields and inverse slopes}

\section{Coalescence parameter: $B_2$}

With a very low binding energy 
($\Delta E = 2.24$ MeV), the (anti-)deuteron is a very loosely bound 
state. Thus, it is formed only at a later stage after kinetic freezout; 
the (anti-)proton and (anti-)neutron must be
close in space and tightly correlated in velocity to coalesce. As a result,
(anti-)deuteron  yields are a sensitive measure
of correlations and can be used to determine the space-time evolution
of the system. If (anti-)deuterons
are formed by coalescence of (anti-)protons and (anti-)neutrons 
and the invariant (anti-)deuteron 
yield can be related~\cite{butler} to the primordial nucleon yields by:

\begin{equation}
E_d\frac{d^3N_d}{dp_d^3} = B_2\left(E_p\frac{d^3N_p}{dp_p^3}\right)^2
\label{eq:b2eqn}
\end{equation}

where the deuteron transverse momentum $p_d = 2p_p$, and $B_2$ is the 
coalescence parameter (subscript 2 refers
to the two nucleons in nuclear cluster). In the above
equation there is an implicit assumption that the ratio of (anti-)neutrons 
to (anti-)protons is unity.  Physically the coalescence parameter is a
measure of the source size: $B_2 \propto 1/V$.

\section{Nuclear Modification Factor: $R_{cp}$}
$R_{cp}$ is a very convenient variable, because we take the multiplicity ratios
for central vs most peripheral events cancelling out a lot of systematics 
related to detector efficiencies and other such factors, leading to a 
relatively clean measurement with minimal systematics due to acceptance, 
efficiency issues. 

Measurement of the $R_{cp}$ variable, has yielded some of the most interesting 
results at RHIC. At mid-rapidity, $R_{cp}$ was observed to be 
suppressed at Au + Au collisions at $\sqrt{s_{NN}} = 200$ GeV, which was 
consistent either with prediction of jet suppression due to Quark-Gluon Plasma
(QGP) or with the depletion of low-$x$ partons due to Color-Glass Condensate
(CGC) hypothesis. Run 3 data with d + Au collisions at $\sqrt{s_{NN}} = 200$ 
GeV, indicated a Cronin like enhancement for $R_{cp}$ at mid-rapidity. This
was inconsistent with the CGC hypothesis. Our present analysis seeks to
extend the $R_{cp}$ measurement for charged hadrons to forward rapidity
(approximate pseudorapidity range $1.2<\eta<2.0$) using the Phenix Muon Arms.
Any variation of $R_{cp}$ from Deuteron going side to the Gold going side
from the nominal value of unity would have important implications. Naively 
one would expect $R_{cp}$ at forward rapidities to behave not very differently
from mid-rapidity and show a Cronin enhancement for both Gold going direction 
and for the Deuteron going direction with a slightly greater increase in the 
Deuteron going direction. However, shadowing effects at small-$x$ (where
$x$ is the fraction of the nucleon momentum carried by the parton) could 
lead to a suppression on the Deuteron going side. CGC hypothesis too, would 
lead to a decrease in the number of scattering centers causing suppression.
Other phenomena like ``longitudinal'' Cronin effect --- in which the particles
in the Deuteron going side get an $\eta$ boost due to multiple scattering
--- can also lead to an effective suppression in the Deuteron going side.

Hence, measurement of $R_{cp}$ can help us to get a deeper understanding of the
perennial interplay between Cronin-like enhancements due to multiple 
scattering and depletion of scattering centers due to shadowing-like effects.

\section{Nuclear modification factor: $R_{cp}$}

In the previous chapter we described how we can identify hadrons using the 
PHENIX Muon Arms. In this chapter we shall describe how we can study the 
initial state effects using hadronic probes. This is done by looking at the 
nuclear modification factor $R_{cp}$ in forward and backward directions for 
d+Au collisions at $\sqrt{s_{NN}}=200$ GeV. The nuclear modification factor 
$R_{cp}$ was defined previously in Eq.~\ref{eq:rcp} as the ratio of the 
particle yield in central collisions 
with the particle yield in peripheral collisions, each normalized by number 
of nucleon nucleon inelastic scatterings $N_{coll}$:
\begin{equation}
R_{cp} = \frac{\left( \frac{dN}{d\sigma dp_T} \right)^{Central}/N_{coll}^{Central}}{\left(\frac{dN}{d\sigma dp_T}\right)^{Peripheral}/N_{coll}^{Peripheral}}
\label{eq:rcp}
\end{equation}
A Glauber model~\cite{glauber} and BBC simulation was used to obtain 
$N_{coll}$. $R_{cp}$ is what we get divided by what we expect. By definition, 
processes 
that scale with the number of underlying nucleon-nucleon collisions $N_{coll}$ 
will produce $R_{cp}=1$. If particle production in Heavy Ion Collisions was
simply an incoherent sum of $p$-$p$ collisions, then $R_{cp}$ would be unity.
Any deviation from unity would indicate a different kind of physics. Thus, we 
assume that peripheral collisions are similar to p+p collisions, allowing us
to normalise $R_{cp}$ independent of the p+p reference spectrum. As a result 
many systematics related to detector efficiencies cancel, leading to a 
relatively clean measurement with minimal systematics. By comparing results 
from d+Au collisions with those from Au+Au collisions we can attempt to 
distinguish between effects that could potentially be due to deconfinement, 
versus effects of cold nuclear matter. $R_{cp}$ for hadrons was seen 
to be suppressed at mid-rapidity in Au+Au collisions REFS?. As mentioned in
Chapter 3, this could be explained in either in terms of:
\benn
\item Jet Suppression: energy loss of energetic particles due to dense 
partonic matter formed as a result of deconfinement. This would be mean that
the observed suppression is a final state effect.
\item Color Glass Condensate (CGC): at sufficiently high energies and low
$x$-values (momentum fraction of nucleon carried by the parton) gluon fusion
processes can deplete the number of scattering centers. This can lead to lower
particle multiplicities and hence suppression in $R_{cp}$. This would mean
that the observed suppression is an initial state effect.
\eenn

However no suppression in $R_{cp}$ was observed in the d+Au collisions at 
mid-rapidity. This seems to indicate that that the observed suppression at
mid-rapidity was likely a final state effects. By looking at $R_{cp}$ at 
forward (and backward) rapidities (REF?) we can probe small $x$. The 
North Arm (d going direction) probes low-$x$ partons from the Au nucleus, 
allowing us to study the suppression/shadowing regime. On the other hand, the 
South Arm probes high-$x$ partons from Au, allowing us to study the 
anti-shadowing/Cronin regime.

\be
x=\frac{M_T}{\sqrt{s}}e^{-y}
\label{eq:x_au}
\ee


\be
x=\frac{M_T}{\sqrt{s}}e^{y}
\label{eq:x_d}
\ee


At low x ~ 10-2, a suppression of partons is observed in the nuclear 
wavefunction (shadowing).

This suppressing any hard
process coupling to those
partons relative to point-like
scaling (a = 1).

At high x ~ 10-1, an 
enhancement (anti-shadowing)
may enhance hard processes.

Color Glass Condensate or
Saturation Physics gives a 
universal QCD explanation
for low x shadowing.
As one probes a proton or nucleus at higher momentum transfer (shorter wavelength), there is an enormous growth of low x gluons.
Thus we might expect that saturation or shadowing effects will play a larger role in higher energy collisions sensitive to a similar range of x.



In the 1960s, scattering  experiments were conducted at
the Stanford Linear Accelerator Center (SLAC) in which very high energy 
electron beams were fired on protons. This experiment was similar to 
Rutherford's classic experiment of bombarding a thin gold foil with 
$\alpha$-particles, which revealed
that the atom consisted of a small massive nucleus, which had most of the 
atom's positive charge, and was surrounded by a cloud of electrons. The SLAC 
experiments found that more electrons were scattered with large momentum 
transfers
than expected. This indicated the presence of discrete scattering centers 
inside the proton, very much the same way large scattering angles of the 
$\alpha$-particles indicated the existence of a small and massive nucleus. 
Moreover, the distribution of the scattering data showed `scale-invariance', 
which indicated that these scattering
centers were `point-like' i.e., they did not have any substructure (at least at
the energy scale they were being probed). These were given the generic name: 
partons. This lead to the developement of the parton model by 
Feynman~\cite{hadron} (and also by Bjorken and Paschos~\cite{bjork69}), in 
which the nucleon was envisaged to consist of essentially free point-like 
constituents, the ``partons'', from which the electron scatters incoherently. 
At a more quantitative level 
they also introduced the concept of parton distributions $q_i(x)$, which 
measure the probability of finding a parton of type $i$ in the proton, with a 
momentum fraction $x$ of the proton momentum. In the parton model, these 
parton distributions are independent of the energy scale at which the proton 
is being probed. 
The data also indicated that the charged scattering centers were spin 
$\frac{1}{2}$ fermions. Subsequently, they were identified with the quarks
proposed by Murray Gell-Man~\cite{gell64}. Later experiments with neutrinos 
also supported this view. We shall however, deal only with electromagnetic 
scattering.

Parton distributions are essential for a detailed understanding of the proton 
structure as well as the planning and interpretation of the High Physics 
experiments in $\bar{p}p$ and $pp$ colliders at Tevatron and LHC. A complete 
description of short-distance scattering experiments involving hadronic 
initial states, 
requires two ingredients from outside perturbative QCD (pQCD) --- the running 
coupling constant $\alpha_{s}(Q^2)$, and the parton distribution 
functions of the nucleon at an input scale $Q^2_0$ . 


==> cpt_theory_akp_phd.tex <==
\chapter{The PHENIX Detector}
In this chapter we shall give an overview of the PHENIX detector as well as 
the subsystems that were used for deuteron/anti-deuteron measurement.

\section{Some jargon}
The field of the relativistic heavy ion physics is saturated with jargon, a 
minefield for the uninitiated. Here is a brief description of some of the
commonly used terms:
\bitm
\item{\bf Central of mass energy:} a.k.a. $\sqrt{s}$, this is the Lorentz
invariant quantity:
\be
s = (p_1+p2)_\mu(p_1+p2)^\mu
\label{eq:s_def1}
\ee 
For nuclei with energy $E_i$ and 3-momentum $\mathbf{p_i}$, it reduces to:

\be
\sqrt{s} = \sqrt{m_1^2+2E_1E_2-2\mathbf{p_1.p_2}+\mathbf{m_2^2}}
\label{eq:s_def2}
\ee
For instance at RHIC (Run 2 and 3), the center-of-mass energy per nucleon is 
$\sqrt{s_{NN}}=200$ GeV. 
\item {\bf Tranverse momentum $p_T$:} this is simply the projection of a 
particle's momentum perpendicular to the collision axis ($z$-axis). 
\be
p_T = p\sin\theta
\label{eq:pt_def}
\ee
where $\theta$ is the polar angle along the $z$-axis. A common variable derived
from this is the transverse energy (or mass) $m_T=\sqrt{p_T^2+m_0^2}$.
\item {\bf Rapidity $y$:} this defines the longitudinal motion scale for a 
particle of mass $m_0$ moving along $z$-axis (the beam axis):
\be
y = \frac{1}{2}\log \left( \frac{E+p_z}{E-p_z} \right)
\label{eq:y_def}
\ee
Since there is cylindrical symmetry around the collision axis, this allows us 
to describe the 4-momentum of particle in terms of its 
transverse momentum $p_T$, rapidity $y$ and the transverse energy $m_T$ as:
\be
p^{\mu}=(m_T \cosh y, p_T \cos \phi_0, m_T\sinh y)
\label{eq:4momentum}
\ee

\item {\bf Pseudorapidity $\eta$:} derived from rapidity (Eq.~\ref{y_def}),
this variable is used when the particle in question is unidentified i.e., $m_0$
is not known:
\be
y = -\log \left( \tan\frac{\theta}{2} \right)
\label{eq:eta_def}
\ee
Where $\theta$ is the angle w.r.t. the beam axis. $\eta$ is often used to 
describe geometrical acceptances of detectors.
\item {\bf Invariant yield:} the
invariant differential cross section of a particle is the probability of 
obtaining $d^3N$ particles in the phase space volume $dp^3/E$ in a given number
of events $N_{event}$:

\be
\frac{1}{N_{event}}E\frac{d^3N}{dp^3} = \frac{d^3N}{N_{event}p_Tdp_Tdy} 
\label{eq:yield_def}
\ee

In cylindrical coordinates $dp^3=dp_xdp_ydp_z$ reduces to 
$p_Tdp_Td\phi m_t\cosh ydy$. Due to azimuthal symmetry we get a factor of 
$1/2\pi$, resulting in the form:
\be
\frac{1}{N_{event}}E\frac{d^2N}{dp^2}=\frac{d^2N}{2\pi N_{event}p_Tdp_Tdy}
\label{eq:ptspectra}
\ee

Using $dN/p_Tdp_T = dN/m_Tdm_T$, we get our final form:
\be
\frac{1}{N_{event}}E\frac{d^2N}{dp^2}=\frac{d^2N}{2\pi N_{event}m_Tdm_Tdy}
\label{eq:mtspectra}
\ee
\item {\bf Centrality:} when the two nuclei collide, there can be range of
impact parameters. Events with a small impact parameter are known as central
events whereas events with a large impact parameter are called peripheral (see
Figure~\ref{fig:impact_par}), and the variation in impact parameters is 
called centrality.

\begin{figure}[h!]
\bcc
\includegraphics[width=0.5\linewidth]{figures/impact_par.eps}  
\caption{Centrality is related to impact parameter: large impact parameter 
events are called peripheral and small impact parameter events are called 
central.}
\label{fig:impact_par}
\ecc
\end{figure}

\item {\bf Minimum Bias:} this is the collection of events containing all 
possible ranges of impact parameters. This is important so that our data does
not have any bias due to events that might be triggered by specific 
signals e.g. presence of a high $p_T$ particle.
\eitm

\section{Invariant yields and inverse slopes}

\section{Coalescence parameter: $B_2$}

With a very low binding energy 
($\Delta E = 2.24$ MeV), the (anti-)deuteron is a very loosely bound 
state. Thus, it is formed only at a later stage after kinetic freezout; 
the (anti-)proton and (anti-)neutron must be
close in space and tightly correlated in velocity to coalesce. As a result,
(anti-)deuteron  yields are a sensitive measure
of correlations and can be used to determine the space-time evolution
of the system. If (anti-)deuterons
are formed by coalescence of (anti-)protons and (anti-)neutrons 
and the invariant (anti-)deuteron 
yield can be related~\cite{butler} to the primordial nucleon yields by:

\begin{equation}
E_d\frac{d^3N_d}{dp_d^3} = B_2\left(E_p\frac{d^3N_p}{dp_p^3}\right)^2
\label{eq:b2eqn}
\end{equation}

where the deuteron transverse momentum $p_d = 2p_p$, and $B_2$ is the 
coalescence parameter (subscript 2 refers
to the two nucleons in nuclear cluster). In the above
equation there is an implicit assumption that the ratio of (anti-)neutrons 
to (anti-)protons is unity.  Physically the coalescence parameter is a
measure of the source size: $B_2 \propto 1/V$.

\section{Nuclear Modification Factor: $R_{cp}$}
$R_{cp}$ is a very convenient variable, because we take the multiplicity ratios
for central vs most peripheral events cancelling out a lot of systematics 
related to detector efficiencies and other such factors, leading to a 
relatively clean measurement with minimal systematics due to acceptance, 
efficiency issues. 

Measurement of the $R_{cp}$ variable, has yielded some of the most interesting 
results at RHIC. At mid-rapidity, $R_{cp}$ was observed to be 
suppressed at Au + Au collisions at $\sqrt{s_{NN}} = 200$ GeV, which was 
consistent either with prediction of jet suppression due to Quark-Gluon Plasma
(QGP) or with the depletion of low-$x$ partons due to Color-Glass Condensate
(CGC) hypothesis. Run 3 data with d + Au collisions at $\sqrt{s_{NN}} = 200$ 
GeV, indicated a Cronin like enhancement for $R_{cp}$ at mid-rapidity. This
was inconsistent with the CGC hypothesis. Our present analysis seeks to
extend the $R_{cp}$ measurement for charged hadrons to forward rapidity
(approximate pseudorapidity range $1.2<\eta<2.0$) using the Phenix Muon Arms.
Any variation of $R_{cp}$ from Deuteron going side to the Gold going side
from the nominal value of unity would have important implications. Naively 
one would expect $R_{cp}$ at forward rapidities to behave not very differently
from mid-rapidity and show a Cronin enhancement for both Gold going direction 
and for the Deuteron going direction with a slightly greater increase in the 
Deuteron going direction. However, shadowing effects at small-$x$ (where
$x$ is the fraction of the nucleon momentum carried by the parton) could 
lead to a suppression on the Deuteron going side. CGC hypothesis too, would 
lead to a decrease in the number of scattering centers causing suppression.
Other phenomena like ``longitudinal'' Cronin effect --- in which the particles
in the Deuteron going side get an $\eta$ boost due to multiple scattering
--- can also lead to an effective suppression in the Deuteron going side.

Hence, measurement of $R_{cp}$ can help us to get a deeper understanding of the
perennial interplay between Cronin-like enhancements due to multiple 
scattering and depletion of scattering centers due to shadowing-like effects.

\section{Nuclear modification factor: $R_{cp}$}

In the previous chapter we described how we can identify hadrons using the 
PHENIX Muon Arms. In this chapter we shall describe how we can study the 
initial state effects using hadronic probes. This is done by looking at the 
nuclear modification factor $R_{cp}$ in forward and backward directions for 
d+Au collisions at $\sqrt{s_{NN}}=200$ GeV. The nuclear modification factor 
$R_{cp}$ was defined previously in Eq.~\ref{eq:rcp} as the ratio of the 
particle yield in central collisions 
with the particle yield in peripheral collisions, each normalized by number 
of nucleon nucleon inelastic scatterings $N_{coll}$:
\begin{equation}
R_{cp} = \frac{\left( \frac{dN}{d\sigma dp_T} \right)^{Central}/N_{coll}^{Central}}{\left(\frac{dN}{d\sigma dp_T}\right)^{Peripheral}/N_{coll}^{Peripheral}}
\label{eq:rcp}
\end{equation}
A Glauber model~\cite{glauber} and BBC simulation was used to obtain 
$N_{coll}$. $R_{cp}$ is what we get divided by what we expect. By definition, 
processes 
that scale with the number of underlying nucleon-nucleon collisions $N_{coll}$ 
will produce $R_{cp}=1$. If particle production in Heavy Ion Collisions was
simply an incoherent sum of $p$-$p$ collisions, then $R_{cp}$ would be unity.
Any deviation from unity would indicate a different kind of physics. Thus, we 
assume that peripheral collisions are similar to p+p collisions, allowing us
to normalise $R_{cp}$ independent of the p+p reference spectrum. As a result 
many systematics related to detector efficiencies cancel, leading to a 
relatively clean measurement with minimal systematics. By comparing results 
from d+Au collisions with those from Au+Au collisions we can attempt to 
distinguish between effects that could potentially be due to deconfinement, 
versus effects of cold nuclear matter. $R_{cp}$ for hadrons was seen 
to be suppressed at mid-rapidity in Au+Au collisions REFS?. As mentioned in
Chapter 3, this could be explained in either in terms of:
\benn
\item Jet Suppression: energy loss of energetic particles due to dense 
partonic matter formed as a result of deconfinement. This would be mean that
the observed suppression is a final state effect.
\item Color Glass Condensate (CGC): at sufficiently high energies and low
$x$-values (momentum fraction of nucleon carried by the parton) gluon fusion
processes can deplete the number of scattering centers. This can lead to lower
particle multiplicities and hence suppression in $R_{cp}$. This would mean
that the observed suppression is an initial state effect.
\eenn

However no suppression in $R_{cp}$ was observed in the d+Au collisions at 
mid-rapidity. This seems to indicate that that the observed suppression at
mid-rapidity was likely a final state effects. By looking at $R_{cp}$ at 
forward (and backward) rapidities (REF?) we can probe small $x$. The 
North Arm (d going direction) probes low-$x$ partons from the Au nucleus, 
allowing us to study the suppression/shadowing regime. On the other hand, the 
South Arm probes high-$x$ partons from Au, allowing us to study the 
anti-shadowing/Cronin regime.

\be
x=\frac{M_T}{\sqrt{s}}e^{-y}
\label{eq:x_au}
\ee


\be
x=\frac{M_T}{\sqrt{s}}e^{y}
\label{eq:x_d}
\ee


At low x ~ 10-2, a suppression of partons is observed in the nuclear 
wavefunction (shadowing).

This suppressing any hard
process coupling to those
partons relative to point-like
scaling (a = 1).

At high x ~ 10-1, an 
enhancement (anti-shadowing)
may enhance hard processes.

Color Glass Condensate or
Saturation Physics gives a 
universal QCD explanation
for low x shadowing.
As one probes a proton or nucleus at higher momentum transfer (shorter wavelength), there is an enormous growth of low x gluons.
Thus we might expect that saturation or shadowing effects will play a larger role in higher energy collisions sensitive to a similar range of x.



In the 1960s, scattering  experiments were conducted at
the Stanford Linear Accelerator Center (SLAC) in which very high energy 
electron beams were fired on protons. This experiment was similar to 
Rutherford's classic experiment of bombarding a thin gold foil with 
$\alpha$-particles, which revealed
that the atom consisted of a small massive nucleus, which had most of the 
atom's positive charge, and was surrounded by a cloud of electrons. The SLAC 
experiments found that more electrons were scattered with large momentum 
transfers
than expected. This indicated the presence of discrete scattering centers 
inside the proton, very much the same way large scattering angles of the 
$\alpha$-particles indicated the existence of a small and massive nucleus. 
Moreover, the distribution of the scattering data showed `scale-invariance', 
which indicated that these scattering
centers were `point-like' i.e., they did not have any substructure (at least at
the energy scale they were being probed). These were given the generic name: 
partons. This lead to the developement of the parton model by 
Feynman~\cite{hadron} (and also by Bjorken and Paschos~\cite{bjork69}), in 
which the nucleon was envisaged to consist of essentially free point-like 
constituents, the ``partons'', from which the electron scatters incoherently. 
At a more quantitative level 
they also introduced the concept of parton distributions $q_i(x)$, which 
measure the probability of finding a parton of type $i$ in the proton, with a 
momentum fraction $x$ of the proton momentum. In the parton model, these 
parton distributions are independent of the energy scale at which the proton 
is being probed. 
The data also indicated that the charged scattering centers were spin 
$\frac{1}{2}$ fermions. Subsequently, they were identified with the quarks
proposed by Murray Gell-Man~\cite{gell64}. Later experiments with neutrinos 
also supported this view. We shall however, deal only with electromagnetic 
scattering.

Parton distributions are essential for a detailed understanding of the proton 
structure as well as the planning and interpretation of the High Physics 
experiments in $\bar{p}p$ and $pp$ colliders at Tevatron and LHC. A complete 
description of short-distance scattering experiments involving hadronic 
initial states, 
requires two ingredients from outside perturbative QCD (pQCD) --- the running 
coupling constant $\alpha_{s}(Q^2)$, and the parton distribution 
functions of the nucleon at an input scale $Q^2_0$ . 


==> dec.tex <==
\newpage
\thispagestyle{empty}
\vspace*{6cm}
{\Large\bf \centerline{Declaration}}
\vspace{1cm}
\noindent
I hereby declare that the work in this thesis is original and has been 
carried out by me under the Ph.D Program, Department of Physics \& Astronomy, 
State University of New York, at Stony Brook under the guidance of Professor
Thomas K. Hemmick and in partial fulfilment of the requirements of the Ph.D 
degree. I further declare that this work has not been 
the basis for the awarding of any degree, diploma or any other title elsewhere.
\begin{flushright}
\vspace{1cm}
Anuj Kumar Purwar\\
SUNY, Stony Brook,\\
July 20, 2004
\end{flushright}
\newpage

